PeRFception: Perception using Radiance Fields

The recent progress in implicit 3D representation, i.e., Neural Radiance Fields (NeRFs), has made accurate and photorealistic 3D reconstruction possible in a differentiable manner. This new representation can effectively convey the information of hundreds of high-resolution images in one compact format and allows photorealistic synthesis of novel views. In this work, using the variant of NeRF called Plenoxels, we create the first large-scale implicit representation datasets for perception tasks, called the PeRFception, which consists of two parts that incorporate both object-centric and scene-centric scans for classification and segmentation. It shows a significant memory compression rate (96.4\%) from the original dataset, while containing both 2D and 3D information in a unified form. We construct the classification and segmentation models that directly take as input this implicit format and also propose a novel augmentation technique to avoid overfitting on backgrounds of images. The code and data are publicly available in https://postech-cvlab.github.io/PeRFception .

==> assets/figures_tex/main/co3d_accuracy.tex <==
\begin{figure}[!tb]
\centering
% \vspace{-4.0mm}
\includegraphics[width=0.90\textwidth]{assets/figures/main/co3d_accuracy.pdf}
\caption{Top-1 and Top-5 accuracy of 3D classification networks trained on \our Co3D dataset. For all networks, spherical harmonic coefficients gives additional cues for 3D object perception}
\label{fig:co3d_accuracy}
% \vspace{-4.0mm}
\end{figure}

==> assets/figures_tex/main/co3d_reconstruction.tex <==
\begin{figure}[!tb]
\centering
\includegraphics[width=0.95\textwidth]{assets/figures/main/co3d_reconstruction.pdf}
\caption{Comparing visual reconstruction quality of original Co3D and our \our Co3D. }
\label{fig:co3d_reconstruction}
\end{figure}

==> assets/figures_tex/main/scannet_semseg.tex <==
\begin{figure*}[!t]
\centering
\includegraphics[width=0.98\textwidth]{assets/figures/main/scannet_semseg.pdf}
% \vspace{-3mm}
\caption{Qualitative results of semantic segmentation on \our ScanNet dataset. (Upper) Ground truth point cloud with ground truth semantic labels, (Bottom) Reconstructed sparse voxels with predicted semantic labels}
\label{fig:scannet_qual}
\end{figure*}

==> assets/tables/main/co3d_benchmark_2d.tex <==

\begin{table}[!t]
\centering
% \refstepcounter{table}
\caption{2D classification accuracies(Acc@1/@5) of the ResNet model trained either on Co3D or \our-Co3D and evaluated either on Co3D or \our-Co3D. [\textbf{P}] denotes the ImageNet\cite{deng2009imagenet} pretrained network.}
\resizebox{.98\textwidth}{!}{
\begin{tabular}{ccccccc}
\toprule
Train Dataset  & \multicolumn{2}{c}{Co3D} & \multicolumn{2}{c}{\our-Co3D (w/o bkgd)} & \multicolumn{2}{c}{\our-Co3D (w/ bkgd)} \\
\cmidrule(lr){1-1} \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
\multicolumn{1}{l}{Test Dataset} & Co3D & \our-Co3D & Co3D & \our-Co3D & Co3D & \our-Co3D  \\ 
\midrule
ResNet18  & 84.69/96.42  & \cellcolor{yellow!40}{80.40/94.41}  & 82.54/95.73  & \cellcolor{yellow!40}{81.63/95.14}  & 83.27/95.59  & \cellcolor{yellow!40}{82.34/95.37} \\
ResNet34  & 86.11/96.72  & \cellcolor{yellow!40}{81.72/94.67}  & 83.90/95.98  & \cellcolor{yellow!40}{82.49/95.51}  & 84.46/96.25  & \cellcolor{yellow!40}{83.62/95.82} \\
ResNet50  & 86.81/96.80  & \cellcolor{yellow!40}{82.17/94.52}  & 83.92/96.12  & \cellcolor{yellow!40}{82.59/95.67}  & 84.93/96.53  & \cellcolor{yellow!40}{83.89/96.04} \\
ResNet101  & 87.47/97.08  & \cellcolor{yellow!40}{82.79/94.85}  & 84.96/96.14  & \cellcolor{yellow!40}{83.66/95.45}  & 85.65/96.63  & \cellcolor{yellow!40}{84.81/96.19} \\
ResNet152  & 87.68/97.11  & \cellcolor{yellow!40}{82.95/94.86}  & 85.23/96.22  & \cellcolor{yellow!40}{84.12/95.67}  & 86.43/96.92  & \cellcolor{yellow!40}{85.27/96.43} \\
ResNext50  & 86.91/96.73  & \cellcolor{yellow!40}{81.96/94.58}  & 84.33/96.07  & \cellcolor{yellow!40}{82.99/95.43}  & 85.34/96.43  & \cellcolor{yellow!40}{84.27/95.85} \\
ResNext101  & 87.75/97.08  & \cellcolor{yellow!40}{82.97/94.88}  & 85.09/95.94  & \cellcolor{yellow!40}{83.96/95.45}  & 86.42/96.71  & \cellcolor{yellow!40}{85.52/96.22} \\
WideResNet50  & 87.36/96.84  & \cellcolor{yellow!40}{82.42/94.65}  & 84.47/96.09  & \cellcolor{yellow!40}{83.26/95.44}  & 85.45/96.37  & \cellcolor{yellow!40}{84.69/96.03} \\
WideResNet101  & 87.71/97.04  & \cellcolor{yellow!40}{83.09/95.02}  & 85.43/96.34  & \cellcolor{yellow!40}{84.12/95.64}  & 86.61/96.83  & \cellcolor{yellow!40}{85.26/96.21} \\
\midrule
ResNet18[P]  & 87.89/97.04  & \cellcolor{yellow!40}{82.91/95.09}  & 85.43/96.44  & \cellcolor{yellow!40}{84.35/95.92}  & 85.98/96.69  & \cellcolor{yellow!40}{84.97/96.15} \\
ResNet34[P]  & 88.80/97.41  & \cellcolor{yellow!40}{84.10/95.23}  & 86.37/96.56  & \cellcolor{yellow!40}{85.48/96.21}  & 87.34/96.91  & \cellcolor{yellow!40}{86.30/96.39} \\
ResNet50[P]  & 89.57/97.56  & \cellcolor{yellow!40}{84.75/95.43}  & 87.44/96.83  & \cellcolor{yellow!40}{86.52/96.38}  & 88.01/97.09  & \cellcolor{yellow!40}{87.38/96.74} \\
ResNet101[P]  & 90.15/97.90  & \cellcolor{yellow!40}{85.44/95.80}  & 88.13/96.90  & \cellcolor{yellow!40}{87.57/96.65}  & 88.90/97.46  & \cellcolor{yellow!40}{88.40/97.10} \\
ResNet152[P]  & 90.74/98.01  & \cellcolor{yellow!40}{86.37/95.95}  & 89.10/97.55  & \cellcolor{yellow!40}{88.15/97.04}  & 89.80/97.74  & \cellcolor{yellow!40}{88.95/97.22} \\
ResNext50[P]  & 89.05/97.46  & \cellcolor{yellow!40}{83.82/95.14}  & 87.34/96.67  & \cellcolor{yellow!40}{86.08/96.06}  & 84.48/96.30  & \cellcolor{yellow!40}{87.21/96.68} \\
ResNext101[P]  & 90.50/97.69  & \cellcolor{yellow!40}{85.80/95.42}  & 88.78/96.87  & \cellcolor{yellow!40}{87.79/96.58}  & 89.20/97.28  & \cellcolor{yellow!40}{88.29/96.86} \\
WideResNet50[P]  & 89.71/97.54  & \cellcolor{yellow!40}{84.66/95.30}  & 87.96/96.62  & \cellcolor{yellow!40}{86.95/96.30}  & 88.17/97.13  & \cellcolor{yellow!40}{87.41/96.72} \\
WideResNet101[P]  & 90.50/97.86  & \cellcolor{yellow!40}{85.84/95.64}  & 88.56/97.02  & \cellcolor{yellow!40}{87.59/96.60}  & 89.05/97.43  & \cellcolor{yellow!40}{88.30/97.06} \\

\bottomrule
\end{tabular}
}
\label{tab:main_co3d_2d}
\end{table}


\begin{comment}
\begin{table}[t]
\centering
% \refstepcounter{table}
\caption{2D classification accuracies(Acc@1/@5) of the ResNet18 model trained either on Co3D or \our-Co3D and evaluated either on Co3D or \our-Co3D. [\textbf{P}] denotes the ImageNet\cite{deng2009imagenet} pretrained network.}
% \vspace{-3mm}
\resizebox{.9\textwidth}{!}{
\begin{tabular}{c|c|c|c|c}
Test Dataset                       & \multicolumn{2}{c|}{Co3D} & \multicolumn{2}{c}{\our-Co3D}  \\ 
\hline
\multicolumn{1}{l|}{Train Dataset} & Co3D & \our-Co3D          & Co3D & \our-Co3D               \\ 
\hline
ResNet  &  72.53/80.29  & \cellcolor{yellow!40}{70.23/79.14}  & 69.65/79.10 & \cellcolor{yellow!40}{71.34/79.75} \\ 
\hline
ResNet[P]  & 84.87/94.42 & \cellcolor{yellow!40}{81.77/92.67}  & 81.29/93.28 &  \cellcolor{yellow!40}{84.33/93.80}
\end{tabular}
}
% \vspace{-3mm}
\label{tab:main_co3d_2d}
\end{table}
\end{comment}

==> contents/main/checklist.tex <==
\section*{Checklist}

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{\revision{Refer to the last page of our main paper.}}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{Refer to the appendix on the supplementary materials.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments (e.g. for benchmarks)...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{The code and data will be publicly available and all the instructions will be provided.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See Section4 and appendix for details.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{Full score tables are in the appendix.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See the appendix.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{Our source datasets(Co3D and ScanNet) and perception models are all cited.}
  \item Did you mention the license of the assets?
    \answerYes{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerYes{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

